Space-time Neural Irradiance Fields for Free-Viewpoint Video

We present a method that learns a spatiotemporal neural irradiance field for dynamic scenes from a single video. Our learned representation enables free-viewpoint rendering of the input video. Our method builds upon recent advances in implicit representations. Learning a spatiotemporal irradiance field from a single video poses significant challenges because the video contains only one observation of the scene at any point in time. The 3D geometry of a scene can be legitimately represented in numerous ways since varying geometry (motion) can be explained with varying appearance and vice versa. We address this ambiguity by constraining the time-varying geometry of our dynamic scene representation using the scene depth estimated from video depth estimation methods, aggregating contents from individual frames into a single global representation. We provide an extensive quantitative evaluation and demonstrate compelling free-viewpoint rendering results.

==> figure/fig_ablation.tex <==
\begin{figure*}[t!]
\begin{center}
\jbox{\linewidth}{0.5\linewidth}
\end{center}
\caption{
\tb{Qualitative comparisons of the variants of our model.}
We show the results from the variants of our model with different loss combinations using the ``CVD'' dataset.
\changil{Each row shows one video; each column shows one variant. Each cell contains a new view synthesis result in addition to potentially several close-ups.}
}
\label{fig:ablation}
\end{figure*}



==> figure/fig_multi_frames.tex <==
\begin{figure}[t]
\begin{center}
\jbox{\linewidth}{0.4\linewidth}
\end{center}
\caption{
\tb{Temporal stability.}
\changil{Show several consecutive frames to demonstrate temporal stability with different models. Add the mesh rendering to show varying disocclusions.}
}
\label{fig:multi_frames}
\end{figure}

==> figure/fig_overview.tex <==
\begin{figure*}[t!]
\begin{center}
\includegraphics[width=.9\linewidth]{figure/image/fig_teaser.pdf}
\end{center}
\caption{
\tb{Overview of the proposed approach.} 
}
\end{figure*}

==> figure/tab_configs_only.tex <==
\begin{center}
\scriptsize
    \begin{tabular}{c|cccccc}
        \hline
        Model & Color & Depth & Empty-space & Static & Flow & Viewing dir. \\
        \hline
        ``NeRF-T'' &&&&&& \\
        A & \checkmark & \checkmark &&&& \\
        B & \checkmark & \checkmark & \checkmark &&& \\
        C & \checkmark & \checkmark & \checkmark & \checkmark && \\
        D & \checkmark & \checkmark & \checkmark & & \checkmark & \\
        E & \checkmark & \checkmark & \checkmark & & \checkmark & \checkmark \\
        F & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \\
        G & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
        \hline
    \end{tabular}
\end{center}


\begin{table*}
\begin{center}
\small
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}ccc@{}}
\toprule
% Model & $\Lcol$ \eqref{eq:color_loss} & $\Ldep$ \eqref{eq:depth_loss} & $\Lfree$ \eqref{eq:zvd_loss} & $\Lstatic$ \eqref{eq:static_loss} & $\Lflow$ \eqref{eq:flow_loss} & Viewing dir. & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
% Model & $\Lcol$ & $\Ldep$ & $\Lfree$ & $\Lstatic$ & $\Lflow$ & V.\ D. & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\multirow{2}{*}{Model} &
\multirow{2}{*}{\parbox{1cm}{\centering $\Lcol$\\\eqref{eq:color_loss}}} &
\multirow{2}{*}{\parbox{1cm}{\centering $\Ldep$ \eqref{eq:depth_loss}}} &
\multirow{2}{*}{\parbox{1cm}{\centering $\Lfree$ \eqref{eq:zvd_loss}}} &
\multirow{2}{*}{\parbox{1cm}{\centering $\Lstatic$ \eqref{eq:static_loss}}} &
\multirow{2}{*}{\parbox{1cm}{\centering $\Lflow$ \eqref{eq:flow_loss}}} &
\multirow{2}{*}{\parbox{1cm}{V.\ D.}} &
\multicolumn{3}{c}{Sintel 1} \\
\cmidrule{8-10}
&&&&&&& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
``NeRF-T'' & \checkmark &&&&& &&& \\
A & \checkmark & \checkmark &&&& &&& \\
B & \checkmark & \checkmark & \checkmark &&& &&& \\
C & \checkmark & \checkmark & \checkmark & \checkmark && &&& \\
D & \checkmark & \checkmark & \checkmark & & \checkmark & &&& \\
E & \checkmark & \checkmark & \checkmark & & \checkmark & \checkmark &&& \\
F & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & &&& \\
G & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &&& \\
\bottomrule
\end{tabular}
\end{center}
\caption{
\tb{Ablation.}
}
\label{tab:ablation}
\end{table*}
